A pair of Second-order complex-valued, N-split operator-splitting methods

The use of operator-splitting methods to solve differential equations is widespread, but the methods are generally only defined for a given number of operators, most commonly two. Most operator-splitting methods are not generalizable to problems with $N$ operators for arbitrary $N$. In fact, there are only two known methods that can be applied to general $N$-split problems: the first-order Lie--Trotter (or Godunov) method and the second-order Strang (or Strang--Marchuk) method. In this paper, we derive two second-order operator-splitting methods that also generalize to $N$-split problems. These methods are complex valued but have positive real parts, giving them favorable stability properties, and require few sub-integrations per stage, making them computationally inexpensive. They can also be used as base methods from which to construct higher-order $N$-split operator-splitting methods with positive real parts. We verify the orders of accuracy of these new $N$-split methods and demonstrate their favorable efficiency properties against well-known real-valued operator-splitting methods on both real-valued and complex-valued differential equations.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{}{}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{A pair of second-order, complex-valued, $\Nop$-split
  operator-splitting methods\thanks{Submitted to the editors DATE.
    \funding{This work was funded by the Natural Sciences and
      Engineering Research Council of Canada through its Discovery
      Grant Program [RGPN-2020-04467] (RJS).}}}

% Authors: full names plus addresses.
\author{Raymond J. Spiteri \thanks{Department of Computer Science,
    University of Saskatchewan, Saskatoon, SK, Canada
    (\email{spiteri@cs.usask.ca}).}  \and Siqi Wei\thanks{Department
    of Mathematics and Statistics, University of Saskatchewan,
    Saskatoon, SK, Canada (\email{siqi.wei@usask.ca})}.}

\usepackage{amsopn}
%\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

